Generative hypergraph clustering: from blockmodels to modularity

Hypergraphs are a natural modeling paradigm for a wide range of complex relational systems. A standard analysis task is to identify clusters of closely related or densely interconnected nodes. Many graph algorithms for this task are based on variants of the stochastic blockmodel, a random graph with flexible cluster structure. However, there are few models and algorithms for hypergraph clustering. Here, we propose a Poisson degree-corrected hypergraph stochastic blockmodel (DCHSBM), a generative model of clustered hypergraphs with heterogeneous node degrees and edge sizes. Approximate maximum-likelihood inference in the DCHSBM naturally leads to a clustering objective that generalizes the popular modularity objective for graphs. We derive a general Louvain-type algorithm for this objective, as well as a a faster, specialized "All-Or-Nothing" (AON) variant in which edges are expected to lie fully within clusters. This special case encompasses a recent proposal for modularity in hypergraphs, while also incorporating flexible resolution and edge-size parameters. We show that AON hypergraph Louvain is highly scalable, including as an example an experiment on a synthetic hypergraph of one million nodes. We also demonstrate through synthetic experiments that the detectability regimes for hypergraph community detection differ from methods based on dyadic graph projections. We use our generative model to analyze different patterns of higher-order structure in school contact networks, U.S. congressional bill cosponsorship, U.S. congressional committees, product categories in co-purchasing behavior, and hotel locations from web browsing sessions, finding interpretable higher-order structure. We then study the behavior of our AON hypergraph Louvain algorithm, finding that it is able to recover ground truth clusters in empirical data sets exhibiting the corresponding higher-order structure.

==> dgleich-extra.tex <==
\usepackage{ushort}
\newcommand{\cel}[1]{\ushort{#1}}
\newcommand{\cbmat}[1]{\left\{ \begin{matrix} #1 \end{matrix} \right\}}
\newcommand{\csbmat}[1]{\left\{\! \begin{smallmatrix} #1
\end{smallmatrix} \! \right\}}
%\newcommand{\csbmat}[1]{\underline{\sbmat{#1}}}
\newcommand{\smallmath}[1]{\begin{smallmatrix}#1\end{smallmatrix}}
\newcommand{\celm}[1]{\cel{\mat{#1}}}
\newcommand{\celv}[1]{\cel{\vec{#1}}}



\newcommand{\calpha}{\ensuremath{\cel{\alpha}}}
\newcommand{\cbeta}{\ensuremath{\cel{\beta}}}
\newcommand{\clambda}{\ensuremath{\cel{\lambda}}}

\newcommand{\cone}{\ensuremath{\cel{1}}}
\newcommand{\ca}{\ensuremath{\cel{a}}}
\newcommand{\cb}{\ensuremath{\cel{b}}}
\newcommand{\cc}{\ensuremath{\cel{c}}}
\newcommand{\cd}{\ensuremath{\cel{d}}}
\newcommand{\ce}{\ensuremath{\cel{e}}}
\newcommand{\cf}{\ensuremath{\cel{f}}}
\newcommand{\cg}{\ensuremath{\cel{g}}}
\newcommand{\ch}{\ensuremath{\cel{h}}}
\newcommand{\ci}{\ensuremath{\cel{i}}}
\newcommand{\cj}{\ensuremath{\cel{j}}}
\newcommand{\ck}{\ensuremath{\cel{k}}}
\newcommand{\cl}{\ensuremath{\cel{l}}}
\newcommand{\cm}{\ensuremath{\cel{m}}}
\newcommand{\cn}{\ensuremath{\cel{n}}}
\newcommand{\co}{\ensuremath{\cel{o}}}
\newcommand{\cp}{\ensuremath{\cel{p}}}
\newcommand{\cq}{\ensuremath{\cel{q}}}
%\newcommand{\cr}{\ensuremath{\cel{r}}}
\newcommand{\cs}{\ensuremath{\cel{s}}}
\newcommand{\ct}{\ensuremath{\cel{t}}}
\newcommand{\cu}{\ensuremath{\cel{u}}}
\newcommand{\cv}{\ensuremath{\cel{v}}}
\newcommand{\cw}{\ensuremath{\cel{w}}}
\newcommand{\cx}{\ensuremath{\cel{x}}}
\newcommand{\cy}{\ensuremath{\cel{y}}}
\newcommand{\cz}{\ensuremath{\cel{z}}}


\newcommand{\cA}{\ensuremath{\cel{A}}}
\newcommand{\cB}{\ensuremath{\cel{B}}}
\newcommand{\cC}{\ensuremath{\cel{C}}}
\newcommand{\cD}{\ensuremath{\cel{D}}}
\newcommand{\cE}{\ensuremath{\cel{E}}}
\newcommand{\cF}{\ensuremath{\cel{F}}}
\newcommand{\cG}{\ensuremath{\cel{G}}}
\newcommand{\cH}{\ensuremath{\cel{H}}}
\newcommand{\cI}{\ensuremath{\cel{I}}}
\newcommand{\cJ}{\ensuremath{\cel{J}}}
\newcommand{\cK}{\ensuremath{\cel{K}}}
\newcommand{\cL}{\ensuremath{\cel{L}}}
\newcommand{\cM}{\ensuremath{\cel{M}}}
\newcommand{\cN}{\ensuremath{\cel{N}}}
\newcommand{\cO}{\ensuremath{\cel{O}}}
\newcommand{\cP}{\ensuremath{\cel{P}}}
\newcommand{\cQ}{\ensuremath{\cel{Q}}}
\newcommand{\cR}{\ensuremath{\cel{R}}}
\newcommand{\cS}{\ensuremath{\cel{S}}}
\newcommand{\cT}{\ensuremath{\cel{T}}}
\newcommand{\cU}{\ensuremath{\cel{U}}}
\newcommand{\cV}{\ensuremath{\cel{V}}}
\newcommand{\cW}{\ensuremath{\cel{W}}}
\newcommand{\cX}{\ensuremath{\cel{X}}}
\newcommand{\cY}{\ensuremath{\cel{Y}}}
\newcommand{\cZ}{\ensuremath{\cel{Z}}}


\newcommand{\cva}{\ensuremath{\celv{a}}}
\newcommand{\cvb}{\ensuremath{\celv{b}}}
\newcommand{\cvc}{\ensuremath{\celv{c}}}
\newcommand{\cvd}{\ensuremath{\celv{d}}}
\newcommand{\cve}{\ensuremath{\celv{e}}}
\newcommand{\cvf}{\ensuremath{\celv{f}}}
\newcommand{\cvg}{\ensuremath{\celv{g}}}
\newcommand{\cvh}{\ensuremath{\celv{h}}}
\newcommand{\cvi}{\ensuremath{\celv{i}}}
\newcommand{\cvj}{\ensuremath{\celv{j}}}
\newcommand{\cvk}{\ensuremath{\celv{k}}}
\newcommand{\cvl}{\ensuremath{\celv{l}}}
\newcommand{\cvm}{\ensuremath{\celv{m}}}
\newcommand{\cvn}{\ensuremath{\celv{n}}}
\newcommand{\cvo}{\ensuremath{\celv{o}}}
\newcommand{\cvp}{\ensuremath{\celv{p}}}
\newcommand{\cvq}{\ensuremath{\celv{q}}}
\newcommand{\cvr}{\ensuremath{\celv{r}}}
\newcommand{\cvs}{\ensuremath{\celv{s}}}
\newcommand{\cvt}{\ensuremath{\celv{t}}}
\newcommand{\cvu}{\ensuremath{\celv{u}}}
\newcommand{\cvv}{\ensuremath{\celv{v}}}
\newcommand{\cvw}{\ensuremath{\celv{w}}}
\newcommand{\cvx}{\ensuremath{\celv{x}}}
\newcommand{\cvy}{\ensuremath{\celv{y}}}
\newcommand{\cvz}{\ensuremath{\celv{z}}}

\providecommand{\cmA}{\ensuremath{\celm{A}}}
\providecommand{\cmB}{\ensuremath{\celm{B}}}
\providecommand{\cmC}{\ensuremath{\celm{C}}}
\providecommand{\cmD}{\ensuremath{\celm{D}}}
\providecommand{\cmE}{\ensuremath{\celm{E}}}
\providecommand{\cmF}{\ensuremath{\celm{F}}}
\providecommand{\cmG}{\ensuremath{\celm{G}}}
\providecommand{\cmH}{\ensuremath{\celm{H}}}
\providecommand{\cmI}{\ensuremath{\celm{I}}}
\providecommand{\cmJ}{\ensuremath{\celm{J}}}
\providecommand{\cmK}{\ensuremath{\celm{K}}}
\providecommand{\cmL}{\ensuremath{\celm{L}}}
\providecommand{\cmM}{\ensuremath{\celm{M}}}
\providecommand{\cmN}{\ensuremath{\celm{N}}}
\providecommand{\cmO}{\ensuremath{\celm{O}}}
\providecommand{\cmP}{\ensuremath{\celm{P}}}
\providecommand{\cmQ}{\ensuremath{\celm{Q}}}
\providecommand{\cmR}{\ensuremath{\celm{R}}}
\providecommand{\cmS}{\ensuremath{\celm{S}}}
\providecommand{\cmT}{\ensuremath{\celm{T}}}
\providecommand{\cmU}{\ensuremath{\celm{U}}}
\providecommand{\cmV}{\ensuremath{\celm{V}}}
\providecommand{\cmW}{\ensuremath{\celm{W}}}
\providecommand{\cmX}{\ensuremath{\celm{X}}}
\providecommand{\cmY}{\ensuremath{\celm{Y}}}
\providecommand{\cmZ}{\ensuremath{\celm{Z}}}

\newcommand{\cmPt}{\cel{\mat{\tilde{P}}}}
\renewcommand{\cmPt}{\mat{\tilde{P}}}

\newcommand{\elm}[1]{\cel{#1}}
